MatSynth: A Modern PBR Materials Dataset

We introduce MatSynth, a dataset of 4,000+ CC0 ultra-high resolution PBR materials. Materials are crucial components of virtual relightable assets, defining the interaction of light at the surface of geometries. Given their importance, significant research effort was dedicated to their representation, creation and acquisition. However, in the past 6 years, most research in material acquisiton or generation relied either on the same unique dataset, or on company-owned huge library of procedural materials. With this dataset we propose a significantly larger, more diverse, and higher resolution set of materials than previously publicly available. We carefully discuss the data collection process and demonstrate the benefits of this dataset on material acquisition and generation applications. The complete data further contains metadata with each material's origin, license, category, tags, creation method and, when available, descriptions and physical size, as well as 3M+ renderings of the augmented materials, in 1K, under various environment lightings. The MatSynth dataset is released through the project page at: https://www.gvecchio.com/matsynth.

==> tables/rebuttal_results.tex <==
\begin{table}
    \centering
    \begin{tabular}{llrr}
        \toprule
        \textbf{Image Type} & \textbf{Metric} & Deschaintre & SurfaceNet \\
        \hline
        \multirow{3}{*}{Renderings} & RMSE & 0.162 & 0.147 \\ 
        & SSIM & 0.540 & 0.544 \\ 
        & LPIPS & 0.351 & 0.346 \\ 
        Diffuse & RMSE & 0.108 & 0.122 \\ 
        Normal & Cos dist & 0.576 & 0.589 \\ 
        Roughness & RMSE & 0.280 & 0.191 \\ 
        Specular & RMSE & 0.095 & 0.076 \\ 
        \bottomrule
    \end{tabular}
    \caption{\textbf{Quantitative results.} Trained on our dataset alone. \vspace{-0.3cm}}
    \label{tab:reb_comparison_quantitative}
\end{table}

